On the Existence of Flight Equilibria in Longitudinal Dynamics

Any control law for aircraft asymptotic stabilization requires the existence of an equilibrium condition, also called trim flight condition. At a constant velocity flight, for instance, there must exist an aircraft orientation such that aerodynamic forces oppose the plane's thrust plus weight, and the torque balance equals zero. A closer look at the equations characterizing the trim conditions point out that the existence of aircraft equilibrium configurations cannot be in general claimed beforehand. By considering aircraft longitudinal linear dynamics, this paper shows that the existence of flight trim conditions is a consequence of the vehicle shape or aerodynamics. These results are obtained independently from the aircraft flight envelope, and do not require any explicit expression of the aerodynamics acting on the vehicle.

==> header.tex <==

\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}

\usepackage{color,graphicx}
\usepackage{subfig}

\usepackage{ae,aecompl,bm}
\let\proof\relax
\let\endproof\relax
\usepackage[cmex10]{amsmath} % assumes amsmath package installed

\usepackage[stable]{footmisc}

% \usepackage[noadjust]{cite}
% \usepackage[sort]{natbib}
\renewcommand{\cite}{\citep}

\usepackage{enumitem,url,theorem}
\usepackage{IEEEtrantools,mathtools}
\usepackage{algorithm,algorithmic}

